Fault-tolerant Consensus in Anonymous Dynamic Network

This paper studies the feasibility of reaching consensus in an anonymous dynamic network. In our model, $n$ anonymous nodes proceed in synchronous rounds. We adopt a hybrid fault model in which up to $f$ nodes may suffer crash or Byzantine faults, and the dynamic message adversary chooses a communication graph for each round. We introduce a stability property of the dynamic network -- $(T,D)$-dynaDegree for $T \geq 1$ and $n-1 \geq D \geq 1$ -- which requires that for every $T$ consecutive rounds, any fault-free node must have incoming directed links from at least $D$ distinct neighbors. These links might occur in different rounds during a $T$-round interval. $(1,n-1)$-dynaDegree means that the graph is a complete graph in every round. $(1,1)$-dynaDegree means that each node has at least one incoming neighbor in every round, but the set of incoming neighbor(s) at each node may change arbitrarily between rounds. We show that exact consensus is impossible even with $(1,n-2)$-dynaDegree. For an arbitrary $T$, we show that for crash-tolerant approximate consensus, $(T,\lfloor n/2 \rfloor)$-dynaDegree and $n > 2f$ are together necessary and sufficient, whereas for Byzantine approximate consensus, $(T,\lfloor (n+3f)/2 \rfloor)$-dynaDegree and $n > 5f$ are together necessary and sufficient.

==> app.tex <==
\section{Proof of Lemma \ref{lem:Z-byz}}
\label{app:Z-byz}

\begin{proof}
    We first prove the following induction statement: $P(k)$ states that $Z_{\min}^{(k)}(v)\in[0,\frac{1}{2}]$ and $Z_{\max}^{(k)}(v)\in[\frac{1}{2},1]$ for all $k\geq 1$. 
    
    In base case when $k=1$, $Z_{\min}(v)\in[0,\frac{1}{2}]$ and $Z_{\max}(v)\in[\frac{1}{2},1]$. Suppose $P(k)$ is true, then
    \[
    Z_{\min}^{(k+1)}(v) = \frac{Z_{\min}^{(k)}(v)}{2} \leq \frac{1}{4},
    \quad
    Z_{\max}^{(k+1)}(v) = \frac{1+Z_{\max}^{(k)}(v)}{2} \geq \frac{3}{4},
    \]
    Hence $P(k+1)$ is also true. Lemma \ref{lem:Z-byz} trivially follows from this statement.
\end{proof}


%\section{Proof of Theorem \ref{thm:RandCR}}
%\label{app:thm:RandCR}

\section{Correctness of RandCR}
\label{app:randCR}

We prove the RandCR is correct. The proof is inspired by prior works \cite{Ben-Or_PODC1983,RP_Aspnes_2002}, and has a similar structure. We include it for completeness. Validity is obvious owing to assumption on crash faults, so we focus on agreement and termination.

\begin{lemma}
    \label{lem:random-1}
    Fix phase $p$. For all nodes that have set the stage-2 state $w_i$ to a non-negative value (in $\{0,1\}$) in phase $p$, they have the same stage-2 state.
\end{lemma}



\begin{proof}
    Recall that in Algorithm RandCR, each node updates phase and stage-1 state atomically (line 3--7 and line 14--21). This implies that once the stage-1 local state $v_i$ of some node $i$ is updated, $i$ proceeds to the next stage. Therefore, the stage-1 state of node $i$ in each phase is a fixed value if it has ever updated it. This allows us to define $C(p)$ as the multiset of stage-1 states of nodes in phase $p$ (excluding those nodes skipping phase $p$). Then, for each node $i$ in phase $p$, $R_i$ is a subset of $C(p)$. Hence, the majority of all non-negative values in $C(p)$ is unique, which proves the lemma. 
\end{proof}

\begin{theorem}
    \label{thm:random}
    Algorithm RandCR (Algorithm \ref{alg:random}) satisfies agreement. 
\end{theorem}

\begin{proof}
    Suppose phase $p$ is the lowest phase in which some node, say $i$, decides its output value $o_i=o$. By Lemma \ref{lem:random-1}, the majority of all stage-1 value in phase $p$ is unique for all nodes. Therefore, if there exists another node $j$ that also decides its output $o_j$ in phase $p$, then $o_j=o_i=o$.
    
    Consider the outputs in a higher phase. By line 17, at least $f+1$ nodes in phase $p$ has stage-2 states $o$. Since there are at most $f$ crashed nodes, all nodes that update to phase $p+1$ without jumping (line 14-21)
    
    must receive at least one phase-$p$ stage-2 state equal to $o$ in their $S$ vector. 
    If there are more than one non-negative values in $S$, then they must be $o$ by Lemma \ref{lem:random-1}. Hence, these nodes will update their stage-1 state to $o$ in phase $p+1$. Similarly, if some node jumps to phase $p+1$ (line 4-5), then again they will have new stage-1 state $o$ by a simple induction. 
    
    In conclusion, all nodes have stage-1 state equal to $o$ in phase $p+1$. By construction, no node changes its state. Hence, all nodes that decide their outputs in phase $p+1$ or higher also agree on the output $o$. Therefore, the algorithm achieves exact consensus.
\end{proof}

\begin{theorem}
\label{thm:RandCR}
Algorithm RandCR (Algorithm \ref{alg:random}) satisfies termination, i.e., it terminates with probability 1.
\end{theorem}

%The proof is similar to the one in prior works \cite{Ben-Or_PODC1983,RP_Aspnes_2002}, so we present int Appendix \ref{app:thm:RandCR}.

\begin{proof}
    %In the previous proof, we showed that all nodes terminate once some node decides its output. 
    Consider the probability that some node $i$ decides its output in phase $p$, where $p$ is the lowest phase in which any node terminates. 
    One sufficient condition for $i$ to decide is that all nodes that have not crashed begin phase $p$ have the same state. We argue that the probability of this event occurs is $1$. 
    %Note that in the worst case, the adversary can control the messages each node receives among the $n-f$ stage-1 messages. In that case, $i$ decides its output if and only if all nodes in phase $p$ have the same state. 
    %\lewis{This sentence is not clear. Why do we need this?} \qinzi{We want to compute the probability that some node terminates in phase $p$, and that's equivalent to the probability that all nodes have the same stage-1 state.} \lewis{Check the new explanation.}
    
    The stage-1 states in phase $p$ come from 3 possible sources. First, it might be a state from some other node, i.e., it is an existing phase-$p$ state (line 7). Second, it can be the majority of the configuration $C(p-1)$ (line 16). Third, it can be a randomly generated state by the Flipcoin function (line 20). 
    
    By Lemma \ref{lem:random-1}, majority of $C(p-1)$ is unique for all $i$. 
    %\lewis{So effectively, we can see the first and second type as same type of messages?} 
    %\qinzi{kind of, but not exactly. We don't need to care about type 1 because as long as all type-3 states agree with type-2 majority, the copied type-1 state must also agree. However, if they don't agree, so don't the type-1 states.}
    Denote $r(p)$ as the number of nodes in phase $p$ that obtain their stage-1 states by Flipcoin generator. Then, all stage-1 states in phase $p$ are identical if and only if all the randomly generated states agree with the majority of $C(p-1)$. Hence, the probability that some node decides its output in phase $p$ is:
    \[
    Pr = \left(\frac{1}{2}\right)^{r(p)}
    \]
    
    Note that $r(p)\leq n$, and $Pr\geq \frac{1}{2^n}>0$. Hence, the probability that the algorithm does not terminate is: 
    \[
    \mathbb{P}(\text{not terminate}) = \lim_{p\to\infty}(1-Pr)^p = 0
    \]
    Thus, the algorithm terminates with probability $1$.
\end{proof}


\section{Proof of Lemma \ref{lem:lower-bound-bits}}
\label{app:lem:lower-bound-bits}

\begin{proof}[Proof Sketch]
    %Suppose for node $i$, the progress condition/predicate of $C_i$ requires $C_i$ to flip at least $\lfloor n/2 \rfloor$ bits. By assumption of $C_i$, each bit only records one receiving event from a specific node. Since there are $r < \lfloor n/2 \rfloor$ bits in $C_i$, $C_i$ can never satisfy the termination condition. Hence, $i$ cannot proceed to a higher phase and cannot terminate. 
    
    Since with only $\lfloor n/2 \rfloor$ bits, each node can only observe and record at most $\lfloor n/2 \rfloor$ receiving events.
    Then consider the scenario where all $n$ nodes are crash-prone and no one suffers a permanent crash failure. Then, we can partition the set of $n$ nodes into two subsets $N_1,N_2$ such that $|N_1|,|N_2|\geq \lceil n/2 \rceil$ and there exist node $i,j$ which receive only from $N_1$ and $N_2$ respectively. In this case. node $i$ and $j$ receive no common information, and hence, $\epsilon$-agreement cannot be achieved.
\end{proof}

\section{Proof of Theorem \ref{thm:lower-bound-bit}}
\label{app:thm:lower-bound-bit}

\begin{proof}
    By Lemma \ref{lem:lower-bound-bits}, we can consider the following scenario. There are two groups of nodes $G_0$ and $G_1$, where all nodes in $G_0$ initially have states $0$, and all nodes in $G_1$ initially have states $1$. Then it is possible that all nodes in $G_0$ receive $0$ only, and all nodes in $G_0$ receive $1$ only. By the assumption of the transition function $Z$, all nodes in $G_0$ update to $0$, and all nodes in $G_1$ update to $1$. Hence, the configuration remains unchanged in each phase. In this case, the algorithm cannot reach $\epsilon$-agreement.
\end{proof}

\section{Lower Bound on Number of Nodes}
\label{app:lower-bound-node}

We prove the impossibility of using Reliable-Broadcast protocol \cite{Bracha:1987} in the family of algorithm we consider. We define the Reliable-Broadcast as a communication protocol that satisfies: correctness, non-forgeability, and uniqueness \cite{OR_Dolev_2004,Bracha:1987}.

\begin{itemize}
    \item Correctness: If a fault-free node $i$ Reliable-Broadcast($i,p,v$), then all fault-free nodes will Reliable-Accept($i,p,v$).
    \item Non-forgeability: If a fault-free node $i$ does not Reliable-Broadcast($i,p,v$), then no fault-free nodes will Reliable-Accept($i,p,v$).
    \item Uniqueness: If some fault-free node Reliable-Accept($i,p,v$) and another fault-free node Reliable-Accept($i,p,v'$), then $v=v'$.
\end{itemize}

% \begin{claim}
%     \label{claim:RB-needs-n-f-nodes}
%     Suppose node $i$ Reliable-Broadcast a message $m$, then all fault-free nodes need to store $m$ in persistent storage space. 
% \end{claim}

% % \qinzi{is it possible that node $i$ only sends to $2f+1$ nodes, and all other nodes waits upon receiving $f+1$ identical messages? No: }

% \begin{proof}
%     Since there are $f$ Byzantine nodes, so each node needs to receive $m$ from at least $f+1$ unique nodes in order to Reliable-Accept $m$. Otherwise, it might receive $m'\neq m$ from the $f$ Byzantine nodes and hence Reliable-Accept $m'$, which contradicts the Correctness property of Reliable-Broadcast protocol. 
    
%     Suppose at most $n/2$ nodes 
% \end{proof}

% \qinzi{Maybe we don't even need the following claim because the above claim itself can show that arbitrary phase gap between $G_{\text{\textsc{Fast}}}$ and $G_{\text{\textsc{Slow}}}$ results in unbounded storage.}

% \begin{claim}
% \label{claim:RB-needs-p}
%     Each node in the Iterative Algorithms needs to transmit at least two values: phase number $p$ and local state $v$.
% \end{claim}

% \begin{proof}
%     Suppose in some algorithm, each node doesn't need to transmit phase $p$. Then consider the following scenario. Suppose there is a fast node $i$ such that the delivery from other nodes to $i$ has no delay. The communication between all other nodes are slow and lossy. In this case, node $i$ repeatedly receive the same messages and proceeds to an arbitrarily high phase while all other nodes are in phase $1$. Since the bound of eventual process, $\Delta$, is unknown, it is impossible to define termination phase, $p_{end}$, a priori.  
% \end{proof}

\begin{lemma}
    \label{lem:RB-impossible}
    Under the crash-recovery model with fair-lossy links and $n\leq 5f$, it is impossible to implement the Reliable-Broadcast primitive as transmitting and receiving steps of the Iterative Algorithms.
\end{lemma}

% \qinzi{you can RB more than 1 message. Impossible to RB more than a constant number of messages.}

\begin{proof}[Proof Sketch]
    % Suppose node $i$ Reliable-Broadcast($i,v,p$). Under Byzantine faults, each node needs to receive ($i,p,v$) from at least $f+1$ different nodes in order to Reliable-Accept($i,p,v$). Otherwise, there are $f$ Byzantine nodes which send faulty messages $(i,p,v')$ such that $v'\neq v$. This contradicts the correctness property.
    
    % At any point of time, at most $f$ nodes are Byzantine faulty, and each one can act as a crashed node. Therefore, each fault-free node must be able to update to next phase by receiving from at most $n-f$ nodes. Otherwise, it is possible that a node only receives $n-f$ messages, and cannot proceed to a higher phase. This contradicts the termination property.
    
    
    Consider the following scenario. There are two groups of nodes. Group $G_{\text{\textsc{Fast}}}$ consists of $n-f$ nodes such that there is no delay between each other. Group $G_{\text{\textsc{Slow}}}$ consists of $f$ nodes such that the communication between $G_{\text{\textsc{Fast}}}$ and $G_{\text{\textsc{Slow}}}$ are slow and lossy. 
    
    There is a scenario where all nodes in $G_{\text{\textsc{Slow}}}$ are crashed nodes. Then by the assumption that the algorithm satisfies termination property, the nodes in $G_{\text{\textsc{Fast}}}$ can proceed to $p_{end}$ by only receiving the $n-f$ messages all from $G_{\text{\textsc{Fast}}}$.
    
    % Each node in $G_{\text{\textsc{Fast}}}$ can proceed to higher phase by receiving the $n-f$ messages from $G_{\text{\textsc{Fast}}}$. 
    
    Now consider the following scenario where all nodes are fault-free. Then, $G_{\text{\textsc{Fast}}}$ can proceed to an arbitrary high phase when $G_{\text{\textsc{Slow}}}$ stays in phase $1$. Since the bound of eventual progress, $\Delta$, is unknown, the phase gap between two groups can be arbitrarily large. 
    
    % \lewis{XXX What is $i$?XXX}
    
    % \qinzi{deleted "from node $i$"}
    
    Since there are $f$ Byzantine nodes, each node needs to receive message $m$ from at least $f+1$ unique nodes in order to Reliable-Accept $m$. Otherwise, it might receive $m'\neq m$ from the $f$ Byzantine nodes and hence Reliable-Accept $m'$, which contradicts the Correctness property of Reliable-Broadcast protocol. In other words, there must be at least $f+1$ nodes that stores the message $m$ and repeatedly broadcast it to other nodes.
    
    As $G_{\text{\textsc{Fast}}}$ proceeds to a higher phase, each node in $G_{\text{\textsc{Fast}}}$ periodically Reliable-Broadcasts its current state in each phase. Each node cannot tell which nodes are in the group $G_{\text{\textsc{Fast}}}$, so there exists a scenario where some node $i$ in $G_{\text{\textsc{Slow}}}$ stores the messages from $G_{\text{\textsc{Fast}}}$. Since the phase gap is arbitrary, this requires an unbounded storage space for node $i$ to store all received messages, which contradicts the assumption on the bounded storage space $c$. %that the persistent storage space is pre-allocated before execution. 
    Hence, Reliable-Broadcast protocol is impossible to use in the specific setup.
\end{proof}

% Remark: it turns out that "uniqueness" property is the most essential part to lower $n$. In the Optimal Resilience paper, the key identity to prove $4t+1$ is that even a Byzantine node sends "fixed" message to all other nodes. This is not true if RB doesn't exists. For example, a Byzantine node can send $0$ to me and send $1$ to you. Under a RB protocol that satisfies uniqueness, it must send a fixed message, say $0$, to both you and me.

% Therefore, we only need to show that there exists no RB that satisfies Uniqueness. This might be a little easier to prove.

\begin{theorem}
    In the crash-recovery model with Byzantine faults, $n=5f+1$ is a necessary condition to solve approximate consensus.
\end{theorem}

\begin{proof}[Proof Sketch]
    Suppose $n=5f$. Consider the following scenario. Suppose $f$ nodes are Byzantine, and among the $4f$ fault-free nodes, $2f$ have initial input $0$ and the other $2f$ have input $1$. By Lemma \ref{lem:RB-impossible}, a Byzantine node can send different values to different nodes, i.e., equivocating. 
    
    In phase $1$, all nodes update to the next phase by receiving $n-f=4f$ nodes in phase $1$.  As argued similarly in the previous proof, we only need to consider this case.
    
    Now, for each node $i$ initially at $0$, it receives $2f$ fault-free messages at $0$, $f$ fault-free messages at $1$, and $f$ Byzantine messages at $0$. Node $i$ cannot tell which messages are Byzantine, and there exists a scenario where all $1$'s  are sent by Byzantine faulty nodes. 
    Therefore, node $i$ cannot change its state, since $0$ is the only valid state in all the possible scenarios.
    
    % \lewis{Old one}: Hence, it drops the $f$ $1$'s to get rid of Byzantine faulty values, and the remaining $2f$ values are all $0$'s. In other words, $U_i$, the input of $Z_i$, consists of $0$ only. By the assumption of transition function $Z_i$, $Z_i(U_i)\in\rho(U_i)=\{0\}$. Therefore, each node $i$ updates to state $0$ in phase $2$. \lewis{$\rho(R_i)=\{0\}$ is incorrect. $R_i$ has $1$'s by your definition. It's not $trim(R_i)$.} 
    
    % \qinzi{see my new definition of $Z_i$ and the new edit}
    
    % \lewis{Check \url{http://disc.ece.illinois.edu/publications/podc35-2012-vaidya.pdf} on how I did the impossibility proof in Sec. 5. We don't need to constraint $Z$. We want $Z$ to be as general as possible. I think my new edit provides enough detail.} \qinzi{yes, makes sense.}
    
    
    
    Similarly for the nodes initially at $1$, they receive $2f$ $1$'s, $f$ $0$'s and $f$ Byzantine messages at $1$. Then, they update to $1$ in phase $2$. In this scenario, each node's state remains unchanged in every phase, and thus, the algorithm does not achieve $\epsilon$-agreement.
    % \qinzi{2 explanations: 1) in a general algorithm, each node still drops the top and bottom $f$ values; 2) the outcome of the update function falls in the inputs, i.e., $v_i=f(R_i)$, then $v_i\in\rho(R_i)$. Maybe we can make this as an assumption (so-called cautious approximate function defined in 87 paper). Intuition of 1): we cannot avoid Byzantine faults, even with RB. These Byzantine messages will affect the update function, so we need to drop them.}
    % \qinzi{Update: I put both 1) and 2) as assumptions. See the "Update" part in the family of algorithm.}
\end{proof}

\section{Sample Figures on Progress}
\label{app:eva-progress}

We use a blue line to mark the point when the approximate algorithm reaches agreement. Note that each node does not know that all nodes reach agreement and only outputs a value when the it reaches phase $p_{end}$.



\begin{figure}[H]
    \centering
        
    \includegraphics[width=\linewidth]{fig/algorithm_2_25_12_0.001_9b541bae88344a63875ead4df5dc1fc9_phase.png}
        
    \caption{Real-time Progress of ACR against Phase}
        
\end{figure}

\begin{figure}[H]
    \centering
        
    \includegraphics[width=\linewidth]{fig/algorithm_2_25_12_0.001_9b541bae88344a63875ead4df5dc1fc9_time.png}
        
    \caption{Real-time Progress of ACR against Time}
        
\end{figure}


\begin{figure}[H]
    \centering
        
    \includegraphics[width=\linewidth]{fig/algorithm_3_15_2_0.001_3b26b28e3e4c4df7a1285bc2c09c27eb_phase.png}
        
    \caption{Real-time Progress of BACR against Phase}
        
\end{figure}

\begin{figure}[H]
    \centering
        
    \includegraphics[width=\linewidth]{fig/algorithm_3_15_2_0.001_3b26b28e3e4c4df7a1285bc2c09c27eb_time.png}
        
    \caption{Real-time Progress of BACR against Time}
        
\end{figure}

\begin{figure}[H]
    \centering
        
    \includegraphics[width=\linewidth]{fig/algorithm_4_25_12_0.001_2bb75103e21c45508085cd3a15161410_phase.png}
        
    \caption{Real-time Progress of RandCR against Phase}
        
\end{figure}

\begin{figure}[H]
    \centering
        
    \includegraphics[width=\linewidth]{fig/algorithm_4_25_12_0.001_2bb75103e21c45508085cd3a15161410_time.png}
        
    \caption{Real-time Progress of RandCR against Time}
        
\end{figure}

\begin{figure}[H]
    \centering
        
    \includegraphics[width=\linewidth]{fig/algorithm_1_25_12_0.001_852e3ec9fd034b02845c283281c96f82_phase.png}
        
    \caption{Real-time Progress of AC against Phase}
        
\end{figure}

\begin{figure}[H]
    \centering
        
    \includegraphics[width=\linewidth]{fig/algorithm_1_25_12_0.001_852e3ec9fd034b02845c283281c96f82_time.png}
        
    \caption{Real-time Progress of AC against Time}
        
\end{figure}



\begin{figure}[H]
    \centering
        
    \includegraphics[width=\linewidth]{fig/JACM86_25_4_0.001_4f68aba2a9834f60b97eef6ea7a7073b_phase.png}
        
    \caption{Real-time Progress of JACM86 against Phase}
        
\end{figure}

\begin{figure}[H]
    \centering
        
    \includegraphics[width=\linewidth]{fig/JACM86_25_4_0.001_4f68aba2a9834f60b97eef6ea7a7073b_time.png}
        
    \caption{Real-time Progress of AC against Time}
        
\end{figure}


\begin{figure}[H]
    \centering
        
    \includegraphics[width=\linewidth]{fig/BenOr_12_5_0.001_f88bccd28b9e478db23bd579f279745a_phase.png}
        
    \caption{Real-time Progress of Ben-Or against Phase}
        
\end{figure}

\begin{figure}[H]
    \centering
        
    \includegraphics[width=\linewidth]{fig/BenOr_12_5_0.001_f88bccd28b9e478db23bd579f279745a_time.png}
        
    \caption{Real-time Progress of Ben-Or against Time}
        
\end{figure}

\section{Comparison with Prior Algorithms}
\label{app:eva-compare}

We present the performance of the following two algorithms:

\begin{itemize}
%    \item Algorithm AC: a simple approximate consensus algorithm in the traditional crash fault model with reliable channel. It is a simple adaption of algorithms from \cite{LocalWait,AA_Dolev_1986,AA_nancy}. 
    
    \item Algorithm JACM86 \cite{AA_Dolev_1986}: an approximate consensus algorithm in the traditional Byzantine fault model with reliable channel.
    
    \item Algorithm Ben-Or \cite{Ben-Or_PODC1983}: a randomized consensus algorithm in the traditional crash fault model with reliable channel.
\end{itemize}

To reflect the difference in our algorithms and prior ones, we use different network protocol and architecture. Prior algorithms do not tolerate message losses, so the TCP protocol is most appropriate to ensure the reliable delivery. For our algorithms, the UDP protocol is more appropriate. The prior algorithms require messages to be sent at specified points as dictated by the algorithm (at the beginning of each phase), whereas ours send messages periodically. Therefore, prior algorithms is single-threaded, and our algorithms have a three-thread structure (send, receive, update thread). We believe this design faithfully reflects the design choice of the algorithms.

Figure \ref{f:compare} presents the performance of AC, JACM86, Ben-Or with $n=12$, no packet loss, no added latency. In this case, they outperform our algorithms.


\begin{figure}[H]
    \centering
        
    \includegraphics[width=\linewidth]{fig/AC, JACM86, Ben-Or.png}
        
    \caption{Performance of AC, JACM86, Ben-Or}
    \label{f:compare}
        
\end{figure}

Figure \ref{f:BACR2} shows that BACR is a bit slower than JACM86, but is still comparable.



\begin{figure}[H]
    \centering
        
    \includegraphics[width=\linewidth]{fig/JACM86, BACR_100_ms_delay_no_drop.png}
        
    \caption{Performance of JACM86 vs. BACR with 100ms delay and no packet drop}
    \label{f:BACR2}
        
\end{figure}

Figure \ref{f:RandCR} is very interesting. It shows that RandCR is slower in most of the cases; however, the max is faster and has a smaller variance.


\begin{figure}[H]
    \centering
        
    \includegraphics[width=\linewidth]{fig/Ben-Or, RandCR_100_ms_delay.png}
        
    \caption{Performance of Ben-Or vs. RandCR with 100ms delay and 10\% packet drop for RandCR}
    \label{f:RandCR}
        
\end{figure}

==> review.tex <==
===== Reviews =====

\noindent \textbf{Review 1:}

To begin with, I find that the title does not reflect well the contents of the paper.

The Introduction is very sketchy, and the results are not clearly stated.
For example, there is no mention of the lower bound results proved in the
paper, nor of the simulation results. There is no mention of how many
failures the algorithms tolerate, or if they are optimal in this sense.
Given the many results that the paper announces, it is not clear at all
why simulation results need to be presented, especially with the limited
number of pages available, the cost is even more sketchy description of
the theoretical results.

\qinzi{explained in detail the meaning of each variable in corresponding sections; to do: will also include it in abstract/intro}

It says in the Abstract:
“ We are interested in the consensus algorithms that store small amount of data in the persistent storage and do not rely on the assumption of eventual delivery or failure detector.”
but in fact later on we learn that consensus is not solvable in this model.

\qinzi{not sure what this means...}

The model is not clearly defined.
In the Crash-Recovery Model section, it says that f nodes may crash,
and the rest may crash and recover; this is not clear. Do the rest of the nodes
may also crash without recovering?
Similarly, I could not understand the Byzantine model. What role plays f here? Only f
may have Byzantine behaviour? Etc.
Also C. Eventual Progress Property is unclear.
Some other model assumptions appear later one, e.g. “need to ensure that some steps are executed atomically, i.e., these steps are either all executed or none is executed”

\qinzi{I personally think the model is clear enough; also re-defined and included all assumptions in Sec.II}

“Simulation of reliable communication in our model is possible only if a node is given unbounded persistent storage space.”
Please provide citation for this result.

The definition of the consensus problems are unclear. What is the set of possible input values?
Why are these defined later on?
The outputs of all crash-prone nodes are within $\epsilon$. Why not all outputs?

\qinzi{We don't care about faulty nodes.}

The proofs are difficult to follow, or not at all included. The section on randomized consensus
is so short that consists essentially only of the code of the algorithm.

\qinzi{New proof should be short and concise enough. Moved proof of randomized algorithm to the main body.}

Many  relevant papers are not discussed; here are some quick examples. The core of the
paper describes approximate agreement algorithms, so it is especially important
to compare the algorithms to previous algorithms (in crash or Byzantine failure models). Do
they need very innovative techniques to make them resilient to crash-recovery with small
persistent state?

\qinzi{not sure how to address this part.} \lewis{Yeah, this reviewer doesn't know anything... We can cite all these papers then.}

Hammurabi Mendes, Maurice Herlihy, Nitin H. Vaidya, Vijay K. Garg:
Multidimensional agreement in Byzantine systems. Distributed Comput. 28(6): 423-441 (2015)


Dolev D, Friedman R, Keidar I, Malkhi D: Failure detectorsin omission failure environments. Technical Report 96-1608,Department of Computer Science, Cornell University, Ithaca,New York, September 1996

Romain Boichat, Rachid Guerraoui:
Reliable and total order broadcast in the crash-recovery model. J. Parallel Distributed Comput. 65(4): 397-413 (2005)

Felix C. Freiling, Christian Lambertz, Mila E. Majster-Cederbaum:
Modular Consensus Algorithms for the Crash-Recovery Model. PDCAT 2009: 287-292

Please revise the references carefully, some don’t even include where the paper was published.


\noindent \textbf{Review 2:}

- The paper says that the Byzantine-tolerant algorithm stores (n-f+2) values in persistent storage, which is not clear to me.  To manage the variables R\_i and S\_i, it seems, if I understand correctly, that node i has to store the messages sent by processes in higher phases so that R\_i can be correctly constructed when the phase of node i proceeds.  I recommend the authors to add an explanation about the persistent storage space of the algorithm (to avoid the misunderstanding).

\qinzi{not sure about this}

- Ths assumptions for the lower bounds are not clear to me.  The paper says, in the last part of Section VI-A, that the storage size of persistent storage is bounded by constant c.  So I think that the lower bounds hold under the assumption of the persistent storage size.  But Theorem 11 shows a non-constant lower bound on the storage size, and Theorem 16 assumes the bounded storage size but not restricted to a constant size.  These seem confusing.

\noindent \textbf{Review 3}

First, the contents of this paper are not closed to the main body.
In order to understand the claims of the paper, the appendix is necessary.
This tendency becomes stronger in the latter part of the paper, especially Sections 5, 6, and 7.

\qinzi{rearranged the structure}

Second, the evaluation section (Section 7) lacks discussion of the simulation results.
The authors should discuss the results to state their thoughts and to clarify their contribution.
The section also has no justification for the simulation settings.
Thus, readers don't understand whether the simulation settings are fair and meaningful.

\qinzi{this is a common comment: should we add more details about simulation?} \lewis{Yeah, let's remove the simulation altogether, since we are submitting to an algorithm/theory track, and we will need to do more work to make the simulation section complete.}
